DCFL: Non-IID awareness Data Condensation aided Federated Learning

Federated learning is a decentralized learning paradigm wherein a central server trains a global model iteratively by utilizing clients who possess a certain amount of private datasets. The challenge lies in the fact that the client side private data may not be identically and independently distributed, significantly impacting the accuracy of the global model. Existing methods commonly address the Non-IID challenge by focusing on optimization, client selection and data complement. However, most approaches tend to overlook the perspective of the private data itself due to privacy constraints.Intuitively, statistical distinctions among private data on the client side can help mitigate the Non-IID degree. Besides, the recent advancements in dataset condensation technology have inspired us to investigate its potential applicability in addressing Non-IID issues while maintaining privacy. Motivated by this, we propose DCFL which divides clients into groups by using the Centered Kernel Alignment (CKA) method, then uses dataset condensation methods with non-IID awareness to complete clients. The private data from clients within the same group is complementary and their condensed data is accessible to all clients in the group. Additionally, CKA-guided client selection strategy, filtering mechanisms, and data enhancement techniques are incorporated to efficiently and precisely utilize the condensed data, enhance model performance, and minimize communication time. Experimental results demonstrate that DCFL achieves competitive performance on popular federated learning benchmarks including MNIST, FashionMNIST, SVHN, and CIFAR-10 with existing FL protocol.

==> sec/ack.tex <==
\section*{Acknowledgment}

The preferred spelling of the word ``acknowledgment'' in American English is 
without an ``e'' after the ``g.'' Use the singular heading even if you have 
many acknowledgments. Avoid expressions such as ``One of us (S.B.A.) would 
like to thank $\ldots$ .'' Instead, write ``F. A. Author thanks $\ldots$ .'' In most 
cases, sponsor and financial support acknowledgments are placed in the 
unnumbered footnote on the first page, not here.

% \section*{References and Footnotes}


==> sec/overview.tex <==
\section{Overview of DCFL}
To put it simply, during the implementation of \myAlg, we use CKA to group division clients according to data complementary and guide client selection, then use complement condensed data as auxiliary data to complete clients.

We use Figure \ref{fig::flowchart}  to illustrate the overall design of \myAlg. The execution flow of \myAlg can be divided into six phases:

\textbf{1. Pre-training of the server model and client grouping}. before training, the server sends requests to clients for its’ condensed data and partial model parameters located in the classifier. When the server receives this information, who can use those condensed data for pre-training and use those model parameters for executing the calculation of CKA to get the local data complementary relationships between overall requested clients.

\textbf{2. Participant selection}. the server incorporates an exploration-exploitation mechanism and combines it with clients’ complementary information which is derived from step 1 for client selection.

\textbf{3. Deliver information}. the server sends model parameters to clients who have never been seen before and sends model parameters and complementary condensed data which may be filtered to clients who have taken part in the training process in the past.

\textbf{4. Local update}. clients that participate in training receive the latest model from the server and training based on its private dataset and may plus the additional received condensed datasets derived from complementary ones, and apply the DSA augmentation in the local training process.

\textbf{5. Upload information}. Clients who never take part in training before send condensate data and updated local model back, while clients who have been selected, only send latest local model to the server.

\textbf{6. Model Aggregation}. when clients complete the computation, the server uses FL optimization methods, like FedAvg, FedProx, FedNova, FedDisco, and so on, to aggregate updates from clients.

Thanks to the structured design, it is easy to integrate FL optimization methods (e.g., FedProx, FedNova, FedAvg, FedDisco, Scoffold) and different data set condensation methods (e.g., DC, DSA, DM) into the proposed framework.

==> sec/ref.tex <==
\section*{References}
% \printbibliography[heading=none]
\bibliography{ref}
\bibliographystyle{IEEEtran}

==> tab/acc_table_12_20.tex <==
% Please add the following required packages to your document preamble:
\renewcommand{\arraystretch}{1.5} %控制行高  
\begin{table*}[tp]  
	\centering  
	\fontsize{6}{8}\selectfont  
        \resizebox{\textwidth}{!}{
	\begin{threeparttable}  
            \caption{\centering{Test accuracy of FL methods with different level of non-iid partitioning}}
            \label{tab::performance_comparison}  
            
            \begin{tabular}{*{14}c}  
                    % 命令用来画表格顶部的粗线，下方有少量垂直间距，可以带一个可选参数改变画线的粗细。
                \toprule
      \multirow{2}{*}{ }&
                \multirow{2}{*}{\textbf{Method}}&  
                \multicolumn{4}{c}{$\alpha = 0.5$}&
                    \multicolumn{4}{c}{$\alpha = 0.1$}&
                    \multicolumn{4}{c}{$C_{k}=2$ (pathological Non-IID)}                                 \\    \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
                                   &                                  & MNIST        & Fashion MNIST & SVHN         & CIFAR-10     & MNIST        & Fashion MNIST & SVHN         & CIFAR-10     & MNIST        & Fashion MNIST & SVHN         & CIFAR-10     \\  \cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
\multirow{2}{*}{\textbf{FedAvg}}   & Tradition                        & {\color[HTML]{333333} 97.39±0.18\%}          & {\color[HTML]{333333} 87.19±0.33\%}          & {\color[HTML]{333333} 86.17±0.33\%}          & {\color[HTML]{333333} 49.15±0.94\%}          & {\color[HTML]{333333} 95.03±0.72\%}          & {\color[HTML]{333333} 77.77±1.67\%}          & {\color[HTML]{333333} 68.52±2.25\%}          & {\color[HTML]{333333} 30.24±1.50\%}          & {\color[HTML]{333333} 71.79±3.82\%}          & {\color[HTML]{333333} 54.00±3.68\%}          & {\color[HTML]{333333} 74.03±2.30\%}          & {\color[HTML]{333333} 35.86±2.27\%} \\
                                   & DCFL                             & {\color[HTML]{333333} 98.53±0.08\%}          & {\color[HTML]{333333} 88.88±0.12\%}          & {\color[HTML]{333333} 92.13±0.09\%}          & {\color[HTML]{333333} 63.64±0.41\%}          & {\color[HTML]{333333} 97.72±0.12\%}          & {\color[HTML]{333333} 84.06±0.29\%}          & {\color[HTML]{333333} 87.47±0.33\%}          & {\color[HTML]{333333} 46.86±0.39\%}          & {\color[HTML]{333333} 91.28±2.12\%}          & {\color[HTML]{333333} 67.52±2.27\%}          & {\color[HTML]{333333} 84.46±0.62\%}          & {\color[HTML]{333333} 52.07±0.98\%} \\ \cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
                \morecmidrules\cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
\multirow{2}{*}{\textbf{FedProx}}  & Tradition                        & {\color[HTML]{333333} 97.35±0.17\%}          & {\color[HTML]{333333} 87.58±0.31\%}          & {\color[HTML]{333333} 87.24±0.38\%}          & {\color[HTML]{333333} 49.66±0.86\%}          & {\color[HTML]{333333} 95.19±0.50\%}          & {\color[HTML]{333333} 80.26±1.27\%}          & {\color[HTML]{333333} 80.96±0.98\%}          & {\color[HTML]{333333} 35.23±1.07\%}          & {\color[HTML]{333333} 75.81±3.93\%}          & {\color[HTML]{333333} 57.88±5.10\%}          & {\color[HTML]{333333} 78.28±1.74\%}          & {\color[HTML]{333333} 38.69±1.93\%} \\
                                   & DCFL                             & {\color[HTML]{333333} 98.52±0.05\%}          & {\color[HTML]{333333} 88.85±0.17\%}          & {\color[HTML]{333333} 91.99±0.12\%}          & {\color[HTML]{333333} \textbf{64.53±0.37\%}} & {\color[HTML]{333333} 97.70±0.12\%}          & {\color[HTML]{333333} \textbf{84.30±0.28\%}} & {\color[HTML]{333333} 88.41±0.61\%}          & {\color[HTML]{333333} 48.03±0.99\%}          & {\color[HTML]{333333} \textbf{93.00±1.10\%}} & {\color[HTML]{333333} \textbf{69.66±2.14\%}} & {\color[HTML]{333333} 84.48±0.52\%}          & {\color[HTML]{333333} \textbf{53.15±0.72\%}} \\ \cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
                \morecmidrules\cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
\multirow{2}{*}{\textbf{FedNova}}  & Tradition                        & {\color[HTML]{333333} 97.37±0.16\%}          & {\color[HTML]{333333} 87.21±0.34\%}          & {\color[HTML]{333333} 86.28±0.30\%}          & {\color[HTML]{333333} 49.30±1.04\%}          & {\color[HTML]{333333} 95.68±0.42\%}          & {\color[HTML]{333333} 78.78±1.53\%}          & {\color[HTML]{333333} 65.89±2.86\%}          & {\color[HTML]{333333} 27.57±1.96\%}          & {\color[HTML]{333333} 74.16±5.56\%}          & {\color[HTML]{333333} 57.50±3.54\%}          & {\color[HTML]{333333} 72.46±2.74\%}          & {\color[HTML]{333333} 35.67±2.04\%} \\
                                   & DCFL                             & {\color[HTML]{333333} \textbf{98.56±0.07\%}} & {\color[HTML]{333333} 89.13±0.12\%}          & {\color[HTML]{333333} 92.22±0.20\%}          & {\color[HTML]{333333} 63.11±0.81\%}          & {\color[HTML]{333333} 97.79±0.12\%}          & {\color[HTML]{333333} 84.10±0.49\%}          & {\color[HTML]{333333} 84.26±1.45\%}          & {\color[HTML]{333333} 46.10±0.65\%}          & {\color[HTML]{333333} 90.64±1.50\%}          & {\color[HTML]{333333} 65.69±2.21\%}          & {\color[HTML]{333333} 82.65±2.00\%}          & {\color[HTML]{333333} 50.02±1.11\%} \\  \cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
                \morecmidrules\cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
\multirow{2}{*}{\textbf{FedDisco}} & Tradition                        & {\color[HTML]{333333} 97.44±0.13\%}          & {\color[HTML]{333333} 87.28±0.33\%}          & {\color[HTML]{333333} 86.62±0.38\%}          & {\color[HTML]{333333} 49.86±1.12\%}          & {\color[HTML]{333333} 95.25±0.62\%}          & {\color[HTML]{333333} 77.49±1.74\%}          & {\color[HTML]{333333} 71.77±2.35\%}          & {\color[HTML]{333333} 30.69±1.60\%}          & {\color[HTML]{333333} 76.09±6.85\%}          & {\color[HTML]{333333} 56.52±4.09\%}          & {\color[HTML]{333333} 74.05±2.55\%}          & {\color[HTML]{333333} 34.78±1.80\%} \\
                                   & DCFL                             & {\color[HTML]{333333} 98.55±0.05\%}          & {\color[HTML]{333333} \textbf{89.16±0.09\%}} & {\color[HTML]{333333} \textbf{92.22±0.13\%}} & {\color[HTML]{333333} 63.62±0.61\%}          & {\color[HTML]{333333} \textbf{97.83±0.09\%}} & {\color[HTML]{333333} 83.64±0.38\%}          & {\color[HTML]{333333} \textbf{88.44±0.30\%}} & {\color[HTML]{333333} \textbf{48.08±0.65\%}} & {\color[HTML]{333333} 91.54±1.49\%}          & {\color[HTML]{333333} 66.50±2.27\%}          & {\color[HTML]{333333} \textbf{85.31±0.69\%}} & {\color[HTML]{333333} 50.26±0.69\%} 
                                   
                                   \\ 
                                    \bottomrule
        \end{tabular}  
                
    	\end{threeparttable} 
        }
\end{table*}  

==> tab/acc_table_copy.tex <==
\renewcommand{\arraystretch}{1.5} %控制行高  
\begin{table*}[tp]  
	\centering  
	\fontsize{6}{8}\selectfont  
        \resizebox{\textwidth}{!}{
	\begin{threeparttable}  
            \caption{\centering{Test accuracy of FL methods with different level of non-iid partitioning}}
            \label{tab::performance_comparison}  
            
            \begin{tabular}{*{14}c}  
                    % 命令用来画表格顶部的粗线，下方有少量垂直间距，可以带一个可选参数改变画线的粗细。
                \toprule
       
                    \multirow{2}{*}{ }&
                \multirow{2}{*}{\textbf{Method}}&  
                \multicolumn{4}{c}{$\alpha = 0.5$}&
                    \multicolumn{4}{c}{$\alpha = 0.1$}&
                    \multicolumn{4}{c}{$C_{k}=2$ (pathological Non-IID)} \cr  
                 %作用和cline类似，可以画出比\midrule更加细小的分隔线，上下有少量垂直间距，可以指定横线所在的列，可以带一个参数调整线条粗细。
                    \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
                    
                &&MNIST&Fashion MNIST&SVHN&CIFAR-10&MNIST&Fashion MNIST&SVHN&CIFAR-10&MNIST&Fashion MNIST&SVHN&CIFAR-10
                    \cr  
                % \midrule 
                    \cmidrule(lr){1-1} \cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
       
                    \multirow{4}{*}{\textbf{Tradition}}
                    &FedAvg& 97.39±0.18\% & 86.97±0.34\% & 86.17±0.33\% & 69.00±0.20\% & 95.03±0.72\% & 77.77±1.67\% & 68.52±2.25\% & 53.00±0.10\% & 71.79±3.82\% & 54.00±3.68\% & 74.03±2.30\% & 54.00±0.10\% \cr
       
                &FedProx&97.35±0.17\% & 87.55±0.25\% & 87.24±0.38\% & 68.73±0.20\% & 95.19±0.50\% & 80.26±1.27\% & 80.96±0.98\% & 54.73±0.25\% & 75.81±3.93\% & 57.88±5.10\% & 78.28±1.74\% & 51.73±0.23\%   \cr
       
                &FedNova&97.37±0.16\% & 87.15±0.34\% & 86.28±0.30\% & 69.25±0.18\% & 95.68±0.42\% & 78.78±1.53\% & 65.89±2.86\% & 53.35±0.28\% & 74.16±5.56\% & 57.50±3.54\% & 72.46±2.74\% & 52.35±0.24\% \cr  
       
                &FedDisco&97.44±0.13\% & 87.27±0.30\% & 86.62±0.38\% & 71.77±2.35\% & 95.25±0.62\% & 77.49±1.74\% & 71.77±2.35\% & 55.15±0.28\% & 76.09±6.85\% & 56.52±4.09\% & 74.05±2.55\% & 53.15±0.18\% \cr
       
                  % \midrule 
    
                 \cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
                \morecmidrules\cmidrule(lr){1-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
                   \multirow{4}{*}{\textbf{DCFL}}&
                FedAvg& 98.53±0.08\% & 88.81±0.17\% & 92.13±0.09\% & 75.32±0.13\% & 97.72±0.12\% & 84.06±0.29\% & 87.47±0.33\% & 57.32±0.13\% & 91.28±2.12\% & 67.52±2.27\% & 84.46±0.62\% & 55.32±0.12\%\cr 
       
                &FedProx&98.52±0.05\% & 88.84±0.12\% & 91.99±0.12\% & 76.51±0.12\% & 97.70±0.12\% & 84.30±0.28\% & 88.41±0.61\% & 58.51±0.12\% & 93.00±1.10\% & 69.66±2.14\% & 84.48±0.52\% & 54.51±0.11\% \cr
       
                &FedNova&98.56±0.07\% & 88.81±0.11\% & 92.22±0.20\% & 76.64±0.41\% & 97.79±0.12\% & 84.10±0.49\% & 84.26±1.45\% & 56.64±0.31\% & 90.64±1.50\% & 65.69±2.21\% & 82.65±2.00\% & 54.64±0.21\% \cr  
       
                &FedDisco&98.55±0.05\% & 88.73±0.23\% & 92.22±0.13\% & 75.77±1.32\% & 97.83±0.09\% & 83.64±0.38\% & 88.44±0.30\% & 57.25±0.18\% & 91.54±1.49\% & 66.50±2.27\% & 85.31±0.69\% & 55.25±0.14\%\cr
                    
                    \bottomrule
        \end{tabular}  
                
    	\end{threeparttable} 
        }
\end{table*}  


==> tab/com_table_12_20.tex <==
\renewcommand{\arraystretch}{1.5} %控制行高  
\begin{table*}[tp]  
	\centering  
	\fontsize{6}{8}\selectfont  
        \resizebox{\textwidth}{!}{
	\begin{threeparttable}  
            \caption{\centering{Number of communication rounds to reach a target accuracy for DCFL and other FL optimization methods on SVHN dataset}}
            \label{tab::communication_comparison}  
            
            \begin{tabular}{c|c|ccc ccc ccc}  
                    % 命令用来画表格顶部的粗线，下方有少量垂直间距，可以带一个可选参数改变画线的粗细。
                % \toprule
                \hline
       
                    \multirow{2}{*}{ }&
                    \multirow{2}{*}{\textbf{Method$\backslash$ToA@}}&  
                    \multicolumn{3}{c}{$\alpha = 0.5$}&
                    \multicolumn{3}{c}{$\alpha = 0.1$}&
                    \multicolumn{3}{c}{$C_{k}=2$ (pathological Non-IID)} \cr  
                 %作用和cline类似，可以画出比\midrule更加细小的分隔线，上下有少量垂直间距，可以指定横线所在的列，可以带一个参数调整线条粗细。
                  % \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
                  \cline{3-5} \cline{6-8} \cline{9-11}
                    
                &&ToA@0.86&ToA@0.87&Accuracy&ToA@0.68&ToA@0.72&Accuracy &ToA@0.72&ToA@0.74&Accuracy
                    \cr  
                % \midrule 
                     % \cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
                       \cline{1-2} \cline{3-5} \cline{6-8} \cline{9-11}
                    \multirow{4}{*}{\textbf{Tradition}}
                    &FedAvg& 74 & -  & 86.20\%  & 85 & -  & 68.29\% & 71 & 71 & 74.49\% \cr
       
                &FedProx  &20 & 61 & 87.38 \% & 15 & 26 & 81.54\% & 34 & 36 & 78.03 \%\cr
       
                &FedNova &90 & -  & 86.27 \% & 96 & -  & 68.64\% & 91 & 98 & 74.84\% \cr  
       
                &FedDisco & 42 & -  & 86.49 \% & 57 & 92 & 72.61\% & 70 & 96 & 74.11\% \cr
       
                  % \midrule 
    
              \cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
                \morecmidrules\cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
                
                
                \multirow{4}{*}{\textbf{DCFL}}
                &FedAvg& 4  & 6  & 92.22 \% & 5  & 6  & 87.59\% & 19 & 23 & 84.25\% \cr 
       
                &FedProx&4  & 5  & 92.09 \% & 4  & 5  & 88.64\% & 14 & 19 & 84.28\% \cr
       
                &FedNova& 3  & 6  & 92.33 \% & 12 & 19 & 85.02\% & 27 & 32 & 82.64\% \cr  
       
                &FedDisco & 4  & 6  & 92.42 \% & 4  & 5  & 88.61\% & 18 & 23 & 85.19\%  \cr
                    
                    \bottomrule
                    % \hline
        \end{tabular}  
                
    	\end{threeparttable} 
        }
\end{table*}  

